Integer Division by Constants: Optimal Bounds

The integer division of a numerator n by a divisor d gives a quotient q and a remainder r. Optimizing compilers accelerate software by replacing the division of n by d with the division of c * n (or c * n + c) by m for convenient integers c and m chosen so that they approximate the reciprocal: c/m ~= 1/d. Such techniques are especially advantageous when m is chosen to be a power of two and when d is a constant so that c and m can be precomputed. The literature contains many bounds on the distance between c/m and the divisor d. Some of these bounds are optimally tight, while others are not. We present optimally tight bounds for quotient and remainder computations.

==> divisionresult_multiplyadd.tex <==

\section{Multiply-Add-Divide Results}

Some authors~\cite{Magenheimer:1987:IMD:36177.36189,Robison:2005:NUD:1078021.1078059} have considered the case where we replace the division by a formula of the multiply-add form $\floor((c * n + b)/m)$ for some $b$. The benefit of the multiply-add approach is that it may allow one to pick a smaller value of $c$, compared to the simpler form
$\floor(c * n/m)$.
%The libdivide library makes use for this optimization. We review and extend these results. %In particular, Robison~\cite{Robison:2005:NUD:1078021.1078059} showed that 

\subsection{Multiply-Add Quotient}
\label{sec:multaddquotient}



As in \S~\ref{sec:quotient}
(taking $Q=\division(n,d)$ and $x=c(n+1)d/m$),
we have that
%
$\division(n,d) = \division(c*n +c , m)$ is equivalent to
\begin{eqnarray*}n-\remainder(n,d)  \leq c*(n+1)*d/m  < n - \remainder(n,d) + d. \end{eqnarray*}
Dividing by $n+1$ throughout, we get 
\begin{eqnarray*}(n-\remainder(n,d))/(n+1)  \leq c*d/m  < (n - \remainder(n,d) + d)/(n+1). \end{eqnarray*}
We have that $(n - \remainder(n,d) + d)/(n+1)$ %is smallest when $n$ is as large as possible with $\remainder(n,d) =d-1$. Its value is one.
is 1 whenever $\remainder(n,d) =d-1$.  It can be
no smaller than 1 for any $n$, given that
$\remainder(n,d) \leq d-1$.
%
We have that $(n-\remainder(n,d))/(n+1) $ is largest when $n$ is as large as possible with $\remainder(n,d)=0$: $n=N-\remainder(N,d)$.
%\oweninline{contributing this text.  Maybe a version of it can be used in the similar section 3.}
We repeat our argument from  \S~\ref{sec:quotient} again. Partition the possible numerators into sets 
\begin{eqnarray*}
N_k = \{ n \in [0,N]\,|\,\remainder(n,d)=k\}.\end{eqnarray*}
Fixing $N$ and $d$, we seek the value $n \in [0,N]$ maximizing \begin{eqnarray*}f(n)=(n-\remainder(n,d))/(n+1).\end{eqnarray*}  For $n \in N_k$ we have $f(n)= (n-k)/(n+1) = 1 - (k+1)/(n+1)$ which is maximized for the largest member of $N_k$.  Let $v$ be the largest member of $N_0$; we have $f(v)= v/(v+1)$.  

We see that the values of $n$ in $[N-d+1, N]$ are precisely the maximizing values in each $N_k$.  Among these, we can show $v$ maximizes $f$ as follows.  
\begin{itemize}
\item Consider any $n \in [N-d+1,N]$ with $n > v$.  Write it as $n = v+k$ with $k\geq 1$
and so $\remainder(n,d)=k$ and $f(n) = (v+k-k)/(v+k+1) = v/(v+1+k) < v/(v+1) = f(v)$.
\item Consider any $n \in [N-d+1,N]$ with $n<v$.
Compare $f(n)$ against $f(v-d) = (v-d)/(v-d+1) < f(v)$.  We write $n$ as $v-d+k$, so $\remainder(n,d)$ is again $k$.  We have $f(n)=(v-d+k-k)/(v-d+k+1) = (v-d)/(v-d+1)+k < f(v-d) < f(v)$.  
\end{itemize}
Thus $n=v$ maximizes $f(n)$.


Hence we have the following result.

\begin{theorem}\label{thm:quotientrobison}
Consider an integer divisor $d>0$ and a range of  integer numerators $n\in[0, N]$ where $N\geq d$ is an integer.
We have that $\division(n,d) =\division(c*n +c , m)$ for all integer numerators $n$ in the range  if and only if
\begin{eqnarray*} \left (1-  \frac{1}{N- \remainder(N,d) + 1} \right ) 1/d \leq c/m < 1/d.\end{eqnarray*} 
\end{theorem}

\begin{remark}Robison~\cite{Robison:2005:NUD:1078021.1078059} derived the sufficient condition $(1-1/(N+1)) 1/d  \leq c/m < 1/d$. When $\remainder(N,d)\neq 0$, Robison's bound is suboptimal unlike Theorem~\ref{thm:quotientrobison}.
\end{remark}

\subsection{Multiply-Add Remainder}
We can extend the results from \S~\ref{sec:multaddquotient} to remainders. As in \S~\ref{sec:remainder}, 
we want $\remainder(n,d) = \division(\remainder(c*n +c , m) * d , m)$ which holds  if and only if 
\begin{eqnarray*}
\remainder(n,d) \leq \remainder(c*(n+1)*d/m,d)< \remainder(n,d)+1.
\end{eqnarray*}
By the same argument as in \S~\ref{sec:remainder}, we want to pick
$c\in [0,m)$ and so we must add the constraint that $\division(n,d) =\division(c*n + c , m)$ or equivalently $\division(n,d) =\division(c*(n+1)*d/m , d)$. Indeed, we can add a multiple of $m$ to $c$ without changing the value of $\remainder(c*n +c , m)$.
By Lemma~\ref{lemma:buzz2}, we have that the two constraints are equivalent to $n\leq c*(n+1)*d/m <n+1$ or  $(1-1/(n+1)) m/d \leq c  < m/d$. This condition should hold for all values of $n$ 
 and we let $N$ be the maximal value of $n$ as it provides the tightest bound, so an equivalent expression is  $(1-1/(N+1)) m/d \leq c < m/d$. 
We have derived the following theorem.

\begin{theorem}\label{thm:remainderrobison}
Consider an integer divisor $d>0$ and a range of  integer numerators $n\in[0, N]$ where $N\geq d$ is an integer.
We have that  $\division(n,d) =\division(c*n+c , m)$  and $\remainder(n,d) =\division(\remainder(c*n +c , m) * d , m)$ for all integer numerators $n$ in the range if and only if
\begin{eqnarray*}\left (1-\frac{1}{N+1} \right )1/d \leq c/m<  1/d.\end{eqnarray*}
\end{theorem}



%We can solve for $c$ and $m$. We verify that $c=1$, $m=d$ is always a solution. We want to show that for any $m$ sufficiently large, there is a solution. Letting $K=N- \remainder(N,d) + 1$, we can rewrite the inequalities as \begin{eqnarray*} \left (1 - \frac{1}{K} \right )\frac{m}{d}  \leq c < \frac{m}{d}.\end{eqnarray*}  Pick $c = \ceiling (m/d) - 1$. Then we can verify that as long as  $m \geq K * d$, the pair of inequalities is satisfied. 
%  In particularly, it means that we can pick  $c =  \ceiling (K) - 1$ and $m=K*d$.
% It applies generally (not just to Theorem~\ref{thm:remainderrobison}), as long as $K$ is independent from $m$ and $c$.


    
\subsection{Multiply-Add Check for Divisibility}
\label{sec:multiplyadddivisibililty}

We can extend the result from \S~\ref{sec:divisibililty} with the multiply-add approach.  

Given Theorem~\ref{thm:remainderrobison},  we can check whether $\remainder(n,d) = 0$ by computing 
\begin{eqnarray*}\division(\remainder(c*n+c , m) * d , m) = 0.\end{eqnarray*}
This equation holds if and only if   $\remainder(c*n+c , m)  < m/d$. By the assumption of Theorem~\ref{thm:remainderrobison}, we have that $m/d \leq c$. Thus if $n$ is a multiple of $d$, then we have that $\remainder(c*n +c , m)  < c$.

By Theorem~\ref{thm:remainderrobison}, we have that  $\division(n,d) =\division(c*n+c , m)$. Hence we have that $\division(c*n+c , m) =\division(c*(n - \remainder(n,d))  +c, m)$ since $n$ and $n - \remainder(n,d)$ have the same quotient with respect to $d$.
It follows that $\remainder(c*n +c , m) -\remainder(c*(n - \remainder(n,d))+c, m) = c*\remainder(n,d)$ and therefore $c*\remainder(n,d) \leq \division(c*n +c , m)$.
Thus if $\remainder(c*n+c , m)  < c$, we have  $c*\remainder(n,d) < c$ which implies  $\remainder(n,d) = 0$.

%\remainder(c*n , m) \geq \division(c*n_2 , m)$
\begin{proposition}\label{prop:multiplyadddivisibility}
Consider an integer divisor $d>0$. We have that $d$ divides $n\in[0, N]$  if and only if 
$\remainder(c*n +c, m)  < c$
subject to the condition that
\begin{eqnarray*}\left (1-\frac{1}{N+1} \right )1/d \leq c/m<  1/d.\end{eqnarray*}\end{proposition}

